Discovery of a Faint Old Stellar System at 150 kpc

We report the detection of a faint old stellar system at $(\alpha,\delta)=(194.29^\circ,~34.32^\circ)$ (SDSS J1257+3419), based on the spatial distribution of bright red-giant branch stars in the Sloan Digital Sky Survey Data Release 4. SDSS J1257+3419 has a half-light radius of $38\pm 12$ pc and an absolute integrated $V$-magnitude of $M_V=-4.8^{+1.4}_{-1.0}$ mag at a heliocentric distance of $150\pm 15$ kpc. A comparison between SDSS J1257+3419 and known Galactic halo objects suggests that SDSS J1257+3419 is either (a) a faint and small dwarf galaxy or (b) a faint and widely extended globular cluster. In the former case, SDSS J1257+3419 could represent an entity of a postulated subhalo of the Milky Way. Further photometric and dynamical study of this stellar system is vital to discriminate these possibilities.

==> README <==

						Oct. 17, 2006
Dear Dr. Sneden

Thank you for your email dated Sep. 22 and for sending me the referee's report
on the paper submitted to the ApJ Letters,  "Detection of a New Galactic Old Stellar System at 150 kpc"
by T. Sakamoto and T. Hasegawa (#21044).

We found the referee's comments very helpful and have revised the manuscript accordingly.
We describe below our response to each of his/her comments and
outline the revisions we have made.

We are sending herewith the revised manuscript and three EPS figures to the ApJ Web Peer Review System.???

We hope that the revised paper is now suitable for publication in ApJ Letters.

Yours sincerely,

Tsuyoshi Sakamoto
National Astronomical Observatory
Okayama Astrophysical Observatory
Asakuchi, Okayama 719-0232
Japan
phone:+81-865-44-2155 
fax:+81-865-44-2360
email: sakamtty@cc.nao.ac.jp

%=============================================================================%

We are very grateful to the referee for his/her useful comments and suggestions
that help us to revise many points in the manuscript.
We have taken into account all of his/her comments in the revisions of the manuscript.

We describe below our response to each of his/her commets and outline the revisions we have made.

1. On the title
The referee indicates that a phrase "new Galactic old stellar system" sounds a bit strange.
According to the comment, we change the title into a new title
"Discovery of a Faint old stellar system at 150 kpc".
We also change "a new Galactic old stellar system" into "a faint old stellar system"
in Abstract and Conclusion, correspondingly.
In addition,   we also change the subsection of Section 2 into "Discovery of a faint stellar system".

2. On Abstract
Following the referee's comments, we add the uncertainties of the half-light radius and distance.
We also add "and" between "photometric" and "dynamical"  in last sentence of Abstract.

3. On the expression in the second paragraph of Introduction 
   We add "may" in the last sentence "......dwarf galaxies have still been missed." 

4. On M31 dwarf galaxies with small angular sizes
  We agree to referee's suggestion that the description of 
  M31 satellite reported by Zucker et al. is added into that of MW satellites
  because it emphasizes the existence of missing dwarf galaxies having 
  small angular sizes .
     
We change the the last sentence of the second paragraph of Introduction 
into "However, Galactic dwarf galaxies with physical sizes of $\lesssim$ 100pc at 200 kpc
and M31 dwarf galaxies (Zucker et al. 2004) have an angular size of a few arcmin,
and then their dwarf galaxies may have still been missed."

5. On the description "the outer edge" in the last sentence of Introduction
Following the referee's comment,  we change the phrase into "the outskirts of the Galactic halo".

6.On adding the paper of Girardi et al. (2004) 
We refer this paper when we fit Padova isochrones to the color-magnitude diagram of SDSS J1257+3419.

7.On the last sentence of the third paragraph in Section 2.
In this part, our expression was unclear, in particular for contamination.
To make clear, as the referee indicates, we change into 
"These checks were carried out in order to assess the contribution of
dwarf star contamination (see preceding paragraph).

8. On specifying the range of the metallicities and horizontal branch morphological types 
    for template globular clusters in Section 2.2
    In the first paragraph, we specify the ranges of the values of [Fe/H] and the horizontal-branch ratio.

9.On limits on the value of [Fe/H]
    In addition to its value which obtained from the analysis of RGB's curvature,
  we also limit on the value of [Fe/H] from the horizontal-branch ratio.
   We  estimate the horizontal-branch ratio of SDSS J1257+3419.
   Based on the [Fe/H] vs. horizontal-branch ratio for Galactic globular clusters (Zinn 1993),
  we suggest that SDSS J1257+3419 has metal-poor nature ([Fe/H]<-1.5).
   Thus, the value of [Fe/H] for SDSS J1257+3419 is less than -1.5 and as low as -2.0 or -2.25.
   We add the description of the above discussion to the last part of the first paragraph of Section 2.2.

10. On the description of star formation history in Section 3

In order to make clear the discussion of the star formation history of SDSS J1257+3419,
we separate the sentences to describe the star formation history
and move to last paragraph.
Following the referee's suggestion, we add the discussion of the intermediate-age stars 
in its last sentence of the last paragraph.

